Semi-Supervised Graph-to-Graph Translation

Graph translation is very promising research direction and has a wide range of potential real-world applications. Graph is a natural structure for representing relationship and interactions, and its translation can encode the intrinsic semantic changes of relationships in different scenarios. However, despite its seemingly wide possibilities, usage of graph translation so far is still quite limited. One important reason is the lack of high-quality paired dataset. For example, we can easily build graphs representing peoples' shared music tastes and those representing co-purchase behavior, but a well paired dataset is much more expensive to obtain. Therefore, in this work, we seek to provide a graph translation model in the semi-supervised scenario. This task is non-trivial, because graph translation involves changing the semantics in the form of link topology and node attributes, which is difficult to capture due to the combinatory nature and inter-dependencies. Furthermore, due to the high order of freedom in graph's composition, it is difficult to assure the generalization ability of trained models. These difficulties impose a tighter requirement for the exploitation of unpaired samples. Addressing them, we propose to construct a dual representation space, where transformation is performed explicitly to model the semantic transitions. Special encoder/decoder structures are designed, and auxiliary mutual information loss is also adopted to enforce the alignment of unpaired/paired examples. We evaluate the proposed method in three different datasets.

==> Experiment.tex <==
\section{Experiments}
We perform experiments on three datasets in different scale and with different graph sizes to evaluate the performance and generalization ability of the proposed model architecture. To further test the benefits of dual embedding and the advantage of introducing unpaired graphs, the comparisons are conducted both in fully-supervised scenario and semi-supervised scenario. In this section, we first put forward the setup of datasets and training configurations, followed by the experimental results compared with baseline methods. After that, extensive analysis are performed to study the significance of each component of our approach. 

\subsection{Settings}
\subsubsection{Dataset} 

We conduct experiments on one synthetic dataset, BA~\cite{Guo2018DeepGT}, and two real-world datasets, Dblp~\cite{Tang2008ArnetMinerEA} and Traffic~\footnote{https://data.cityofnewyork.us/Transportation/2018-Yellow-Taxi-Trip-Data/t29m-gskq}. 
\begin{itemize}
    \item \textbf{BA} In BA dataset, source domain are constructed by the Barabasi-Albert model~\cite{McInnes1999EmergenceOS}, a classical random graph generation approach, where each node is connected to one existing node. Each graph is set to have $20$ nodes, and the target graph is constructed as $2$-hop reach-ability graph(e.g. if node i is $2$-hop reachable from node j in the source graph, then they are connected in the target graph). Node attributes are initialized using its connectivity with other nodes.
    
    \item \textbf{Dblp} Dblp is a multi-view citation network, with $22559$ nodes representing researchers. It provides edges of three types, representing co-authorship, citation, and research overlapping respectively. Each node has a $2000$-dimension vector available, encoding the research interests. In our experiment, we use the citation network as the source, and research overlapping network as the target domain. This dataset is given in the transductive learning setting, and all the nodes appeared in one single large graph. Addressing that, we manually split it, by first selecting a center node and then sampling nodes within its 2-hop neighborhood to get a smaller graph. 
    
    \item \textbf{Traffic} For traffic dataset, we use the publicly available New York Taxi Trip dataset in year $2015$. Each trip record contains the take-on and take-off places, as well as the trip-start time. We split the city into $100$ regions, and build the edges based on the taxi flow amount between each region pairs within one hour. This results in $365*24$ graphs in total. On this dataset, we perform a traffic flow prediction task, and set the target domain as the graph state one hour in the future. Node attributes are initialized using the mean of historic taxi flows in the past $24$ hours.
\end{itemize}

\begin{table}[h]
  \centering
  \setlength{\tabcolsep}{4.5pt}
  \normalsize
  \begin{tabular}{ | c | c || c  | c | c |}

    \hline
    \multicolumn{2}{|c||}{} & BA & Dblp & Traffic \\
    \hline
    \multicolumn{2}{|c||}{Dataset Size} & 5000 & 22559 & 8760 \\
    \multicolumn{2}{|c||}{Average graph size} & 20 & 125 & 100 \\
    \multicolumn{2}{|c||}{Dataset type} & Inductive & Transductive  & Inductive \\
    \hline
    Supervised & Paired & 3000 & 13535 & 5256 \\
    \hline
    Semi-sup & Paired & 500 & 2255 & 876 \\
    Semi-sup & Unpaired & 2000 & 9020 & 3504 \\
    \hline
  \end{tabular}
  \label{tab:real}
  \caption{Summarization of the statistics of three datasets. }
  \vskip -0.1in
\end{table}

The overall statistics of these three datasets are summarized in Table 1. 'Dataset Size' means the total number of graphs for inductive dataset, and total number of nodes for transductive dataset. For fully-supervised experiments, the amount of paired graphs used for training are listed in the 'Supervised-Paired' row. For semi-supervised training scenario, the used paired graph and unpaired graph amounts are also listed in the 'Semi-sup-Paired' and 'Semi-sup-Unpaired' respectively.

\subsubsection{Baselines}
Because our goal is to show the benefits of utilizing unpaired graphs and to verify the expressiveness of our model architecture, we make comparisons to two previous approaches, DGT~\cite{Guo2018DeepGT} and NEC-DGT~\cite{Guo2019DeepMG}. NEC-DGT is the state-of-the-art model in graph translation. Both these two approaches can only work with fixed graph sizes, unlike our model, which accepts arbitrary graphs. So, when applying them to Dblp dataset, we change all the training and testing graphs to $100$ nodes, through padding(when the graph is smaller) and down-sampling(when the graph is larger).

For Implementation of these two methods, we directly used their codes from the Github, and modified their dataloader to work with our datasets. Furthermore, we extend NEC-DGT with an auxiliary source-domain decoder to get 'NEC-DGT-Enhanced' model, so that it can utilize unpaired graphs in the source domain. Through comparing with it, we can test the importance of using dual embedding spaces instead of a shared one.


\subsubsection{Configurations}
All experiments are conducted on a $64$-bit machine with Nvidia GPU (Tesla V100, 1246MHz , 16 GB memory), and ADAM optimization algorithm is used to train all the models. 

In fully supervised setting, all models are tested. While in semi-supervised setting, only NEC-DGT-Enhanced and our model are run. Because edges in graphs are usually sparse, we re-weight the importance of edges and non-edges in loss calculation, during both training and testing, to solve this class imbalance problem. For DGT, NEC-DGT, and NEC-DGT-Enhanced, the learning rate is initialized to $0.0001$, following the settings in their code. For our model, the learning rate is initialized to $0.001$. All models are trained until converging, with the maximum training epoch being $5000$. 

For the evaluation metrics, we adopt mean squared error(MSE) and mean average percentage error(MAPE). As MSE is more sensitive when the ground-truth value is large and MAPE is more sensitive when the ground-truth value is small, we believe they can provide a more comprehensive comparison combined. Besides, class-imbalance exists in this problem, as edges are usually sparse, and directly training on them would result in trivial results. Addressing it, we re-weight the importance of edges and non-edges during the loss calculation, in both training and testing. Each experiment is run $5$ times with different random seeds, and both mean and standard deviation of its score are calculated for a fair comparison.


\subsection{Main result}
In this part, we show the comparisons between our model and all baseline approaches. In Table 2, the MSE losses of the translated results are present. In Table 3, the MAPE losses of them are shown.

\textbf{Supervised} In this setting, we utilize a large amount of paired graphs, to evaluate the architecture of our model in capturing the translation pattern. It can be observed that in this case, our model outperforms all other approaches by a large margin. Our approach shows an improvement of $0.082$ on BA dataset, $0.056$ on Dblp, and $0.009$ on Traffic dataset respectively, in term of MSE loss. The results are similar on the MAPE loss. These results validate the effectiveness of our model design. Besides, through the comparison between "NEC-DGT" and "NEC-DGT-enhanced", it also shows that improvements can be gained through utilizing unpaired graphs and introducing auxiliary reconstruction task. A more detailed analysis of this can be found in the ablation study part.

\textbf{Semi-supervised} In the semi-supervised setting, our model also achieves the best performance. It outperforms "NEC-DGT-enhanced" by $0.102$, $0.022$ and $0.012$ points in MSE loss, and $0.093$, $0.013$ and $0.015$ points in MAPE loss, on three datasets. Note that the improvement on Dblp dataset is smaller, and it could results from the dataset size. Dblp dataset is significantly larger than both other two datasets, therefore, the bonus from adding more unpaired graphs is relatively limited. Furthermore, looking at the standard deviations, it can be observed that NEC-DGT-enhanced is more unstable than ours, and getting higher performance variations. This phenomena could result from NEC-DGT-enhanced's difficulty in trading-off between the semantics from source domain and the semantics from target domain in the intermediate embedding space. These results can validate the intuition that explicitly modeling the difference of two domains in the intermediate space can make it easier for the model to utilize unpaired graphs.

\begin{table*}[h]
  \centering
  \setlength{\tabcolsep}{4.5pt}
  \normalsize
  \begin{tabular}{c || c | c || c | c || c | c }

    \hline
    methods &  \multicolumn{2}{|c||}{BA} &  \multicolumn{2}{|c||}{Dblp} &  \multicolumn{2}{|c}{Traffic} \\
    \hline
    & MSE & MAPE & MSE & MAPE & MSE & MAPE \\
    \hline
    DGT & $0.374\pm0.0033$ & $0.279\pm0.0024$ & $0.352\pm0.0074$ & $0.264\pm0.0068$ & $0.248\pm0.0071$ & $0.181\pm0.0063$ \\
    NEC-DGT & $0.213\pm0.0006$ & $0.153\pm0.0004$ & $0.191\pm0.0013$  & $0.142\pm0.0006$ & $0.138\pm0.0274$ & $0.110\pm0.0186$ \\
    NEC-DGT-enhanced & $0.195\pm0.0004 $  & $0.144\pm0.0003 $ & $0.187\pm0.0016$ &  $0.129\pm0.0009$ & $0.076\pm0.0087$  & $0.054\pm0.0066$  \\
    Our model & $\mathbf{0.113\pm0.0028}$  & $\mathbf{0.083\pm0.0019}$ & $\mathbf{0.131\pm0.0007}$ & $\mathbf{0.097\pm0.0003}$ & $\mathbf{0.067\pm0.0046}$ & $\mathbf{0.060\pm0.0027}$ \\
    \hline
  \end{tabular}
  \label{tab:real}
  \caption{Comparison of different approaches in the fully supervised scenario, tested on three datasets. }
  \vskip -0.1in
\end{table*}

\begin{table*}[h]
  \centering
  \setlength{\tabcolsep}{4.5pt}
  \normalsize
  \begin{tabular}{c || c | c || c | c || c | c }

    \hline
    methods &  \multicolumn{2}{|c||}{BA} &  \multicolumn{2}{|c||}{Dblp} &  \multicolumn{2}{|c}{Traffic} \\
    \hline
    & MSE & MAPE & MSE & MAPE & MSE & MAPE \\
        \hline
    NEC-DGT-enhanced & $0.195\pm0.0004 $  & $0.191\pm0.021$ & $0.187\pm0.0016$ & $0.168\pm0.0033$ & $0.076\pm0.0087$  & $0.075\pm0.012$  \\
    Our model &$\mathbf{0.113\pm0.0028}$  & $\mathbf{0.098\pm0.0011}$ & $\mathbf{0.131\pm0.0007}$ & $\mathbf{0.155\pm0.0003}$ & $\mathbf{0.067\pm0.0046}$ & $\mathbf{0.060\pm0.0027}$ \\
    \hline
  \end{tabular}
  \label{tab:real}
  \caption{Comparison of different approaches for three datasets in the semi-supervised scenario.}
  \vskip -0.1in
\end{table*}




\subsection{Case study}
In Figure 5, we provide an example in the BA dataset to show the translation result of our trained model. The upper left is the source graph, upper right is the target graph, and the lower one is the translated result graph. It can be seen that our model captured the pattern behind translation.

\begin{figure}[h!]
  \centering
    
    \includegraphics[height = 40mm,width=40mm]{image_xiang/ori_BA.png}
    \includegraphics[height = 40mm,width=40mm]{image_xiang/tgt_BA.png}
    \includegraphics[height = 40mm,width=40mm]{image_xiang/new_BA.png}
    
    \caption{Obtained Case study examples.}
  \setlength{\abovecaptionskip}{0cm}
\end{figure}

\subsection{Ablation study}
In this subsection, we analyze the importance of each factor in our model.

\textbf{Sensitivity to paired-unpaired ratio}
In this part, we show the sensitivity of our model when changing the amount of paired graphs. As shown in Figure 6, we change the ratio of paired graphs during training from $5$ percent to $30$ percent of total graphs, and record the test MSE loss. When the ratio is less then $8$ percent, the effects of increasing paired graphs is not clear. But when it is between $8$ and $13$ percent, the increase become much sharper. When it is more then $16$ percent, the gaining from adding more paired training examples become smaller again.

\begin{figure}[h!]
  \centering
    
    \includegraphics[height = 40mm,width=60mm]{sensitivityanalysis.pdf}
    
    \caption{Sensitivity analysis over unpaired ratio.}
  \setlength{\abovecaptionskip}{0cm}
\end{figure}




\begin{table}[h]
  \centering
  \setlength{\tabcolsep}{4.5pt}
  \normalsize
  \begin{tabular}{c || c  || c }

    \hline
    methods & BA & Dblp\\
    & Semi sup & Semi sup \\
    \hline
    Shared Embedding & 0.196 & 0.245 \\
    No position & 0.142 & 0.204 \\
    No MI & 0.141 & 0.197  \\
    No multi-head attention & 0.135 & 0.190 \\
    All included & 0.132 & 0.192  \\
    \hline
  \end{tabular}
  \label{tab:real}
  \caption{Evaluation of the significance of different designs in our approach on BA and Dblp datasets. The scores are computed using MSE loss.}
  \vskip -0.1in
\end{table}

\textbf{Gain from dual embedding}
In our model design, so-called 'dual embedding' is adopted to distinguish between the source and the target domain. Explicitly modeling the difference across two domains can ease the trade-off between reconstruction and translation, and help the model to learn more from unpaired graph. In Table 4, it shows that on both BA and Dblp dataset, removing this part and changing to use shared embedding would result in a signicant performance drop, about $0.065$ and $0.053$ points respectively, measured using MSE loss. Besides, we can look at the performance of $NEC-DGT-enhanced$ in Table 2, which also utilize the unpaired graphs through reconstruction task without building two embedding spaces. In the supervised setting, where all training samples are paired, it performs better than 'NEC-DGT'. But when changing to the semi-supervised setting, the performance dropped significantly, and the loss has a large standard deviation. The reason is that the trade-off is more difficult to make when the training samples are limited, and it would result in unstableness during training.

\textbf{Importance of position embedding}
In this part, we test the effects of the position embedding, to test its benefits in guiding the encoding process. The model architecture remains unchanged. We input the first eight dimension of node attributes to replace the calculated position embedding, and check its performance. Through the result in Table 4, it can be seen that it will result in a performance drop of $0.01$ on BA, and $0.012$ on Dblp. This result shows that position embedding is important for extending representation ability of graph encoder module.


\textbf{Importance of MI loss}
We also test the benefits from auxiliary mutual information loss when aligning the transformed embedding of unpaired graphs. For this experiment, we simply remove this loss during the fine-tune steps, and compare the performance change. We find a drop of $0.009$ points on BA, and $0.005$ on Dblp. The drop is smaller on Dblp datast, and it may still be a result of dataset size. As Dblp is much larger, the number of paired graphs is more sufficient for the training, which makes this auxiliary loss not that important. But overall, we can observe that this supervision can train the translator better.


\textbf{Influence of multi-head attention}
In this part, we test the influence of the multi-head attention module in the decoding process. This module is designed to fuse the processed embedding of nodes based on their relative distances. The relative distances is measured using the processed position embedding along with the metric space constructed by each attention head. Through multi-head attention, higher-order interaction between processed node embedding and position embedding is supported. From Table 4, we can see that on BA dataset, this module can bring a moderate improvement of around $0.003$. On Dblp dataset, the performance is similar whether this module is removed or not. 

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> methodology.tex <==
\section{Methodology}
In this section, we formally propose the Dual Embedding Graph Translator(DEGT) for semi-supervised graph translation tasks. First, we present an introduction of the overall framework architecture. Then, we go into details of the design of each componential module. Following that, we elaborate on the adopted training losses, and summarize by providing the full algorithm.

\subsection{Overall Architecture}
The essence of our method is the utilization of mono-domain graphs to provide auxiliary training signals for the learning process. It is a common practice in using reconstruction tasks to improve the quality of obtained intermediate embedding, requiring the encoder to extract complete and representative features. Through sharing the same decoder for both translation and reconstruction tasks, its ability in modeling the graph distribution of the target domain can also be enhanced. Due to the semantic gap issue, instead of constructing one shared embedding space and expect it to be domain-agnostic, we explicitly modeling the semantic transition process through a translator module, and form the so-called 'dual embedding' between the source and target domain.

Composing aforementioned modules together, we obtain the overall architecture of our framework, as shown in Figure 2. The upper branch is the auto-encoder in the source domain, the lower branch is that in the target domain, and their correspondence is built in the intermediate embedding space. In our implementation, the translator is a simple multi-layer perceptron, and the structure of encoder/decoder is specially designed to achieve higher expressive capacity. Furthermore, to align the distribution of two embedding spaces, an auxiliary loss basing on mutual information is used, besides the translation/reconstruction losses. All these parts will be presented in detail in the following subsections.

\begin{figure*}[t!]
  \centering
    
    \includegraphics[height = 80mm,width=162mm]{overall.pdf}
    
    \caption{Overview of the framework}
  \setlength{\abovecaptionskip}{0cm}
\end{figure*}

%graph VAE framework
\subsection{Encoder}
\begin{figure}[t!]
  \centering
    
    \includegraphics[height = 35mm,width=60mm]{encoder.pdf}
    
    \caption{Overview of the encoder}
  \setlength{\abovecaptionskip}{0cm}
\end{figure}
Previous works have found two main issues of classical GNNs. The first is that their expressiveness is significantly constrained by the depth. For example, a k-layer graph convolution network(GCN) can only capture k-order graph moments without the bias term~\cite{dehmamy2019understanding}, and each layer is effectively a low-pass filter and resulting in too smooth graph features as it goes deep~\cite{wu2019simplifying}. The second issue is that most of them are position-agnostic. Classical GNNs fail to distinguish two nodes with similar neighborhood but at different positions in the graph~\cite{you2019position,zhao2019hashing}. This problem becomes severer when we are using GNN to extract node embeddings to predict the existence of edges. %Message passing mechanism functions only at the local level each time. Therefore, although it can fuse the information from distant nodes through stacking, it is still difficult to capture semantic information stored in the global layout.

Addressing them, we extend classical message-passing based GNNs by adding skip connections and using position embeddings, as shown in Figure 3. With skip connections, higher GNN layers can still access lower-level features, and better representations can be learned. As to the position embedding, inspired by the work of ~\cite{you2019position}, we represent each node using the lengths of their shortest paths to a couple of selected anchors. As proven by their work, bound of position distortions can be calculated for an anchor set of the size $O(log^{2}N)$, where $N$ is the number of nodes in that graph. Considering the size of graphs in our dataset, we preset it to eight for simplicity. Concretely, each time one graph is to be inputted, we randomly selected eight nodes as anchors, and calculate position embeddings basing on them. Although the absolute values of obtained position embeddings would be different when the anchor set changes, their relative relationship remains the same, and can be exploited. 
%(Besides, as suggested in [], not-connected is also a form of information. So, we augment the original graph with another adjacency matrix $A^*$, which is the complementary graph of $A$. When node number is very high, it would be a dense graph with many repetitive information. So, we randomly sampling edges in it, assuring that no node has more then five neighbors in $A^*$.)

With these preparations, now we can present the formulations of our extended GNN structure. In $l$-th block, the message passing and fusing process can be written as:
\begin{displaymath}
F_{v}^{l+1}  = \sigma(W_{F} \cdot (F_{v}^{l} \parallel AGG(\{F_{u}^{l}, \mathcal{A}_{u,v}=1\}))) \parallel F_{v}^{0},
\end{displaymath}
\begin{displaymath}
P_{v}^{l+1}  = \sigma(W_{P} \cdot (P_{v}^{l} \parallel AGG(\{P_{u}^{l}, \mathcal{A}_{u,v}=1\}))) \parallel P_{v}^{0}, 
\end{displaymath}
wherein $F_{v}$ refers to the feature embedding of node $v$, and $P_{v}$ refers to its position embedding. $AGG$ aggregates information from nodes neighboring $v$, for which we adopt average function. $\parallel$ means concatenate, $W$ is the weight parameter, and $\sigma$ refers to the activation function. 

\subsection{Decoder}
\begin{figure}[t!]
  \centering
    
    \includegraphics[height = 50mm,width=90mm]{decoder.pdf}
    
    \caption{Overview of the decoder}
  \setlength{\abovecaptionskip}{0cm}
\end{figure}
After the encoding part, for each node $v$, now we have two representation vectors, $F_{v}$ and $P_{v}$. $F_{v}$ is the embedding of the node attributes, and $P_{v}$ is the processed embedding for its relative position in the graph. To predict the existence of edges between two nodes, clearly both these two features are helpful. Considering that these two features carry different-level semantic meanings and are in different embedding spaces, directly concatenating them might be improper. In order to learn to fuse the position and attribute information, we construct the decoder with a number of same-structured blocks. Inside the block, we apply a multi-head attention layer~\cite{vaswani2017attention} with 'Query'/'Key' being $P$ and 'Value' being $F$. Its formulation can be written as:
\begin{displaymath}
Attention(Q,K,V) = softmax(\frac{QK^T}{\sqrt{d_k}}) \cdot V,
\end{displaymath}
\begin{displaymath}
head_i = Attention(PW_i^Q,PW_i^K,FW_i^V),
\end{displaymath}
\begin{displaymath}
H_F = (head_1 \parallel head_2 \parallel ... \parallel head_h) \cdot W^O.
\end{displaymath}
$W_i^Q \in \mathbb{R}^{d_P,d_k}, W_i^K \in \mathbb{R}^{d_P,d_k},  W_i^V \in \mathbb{R}^{d_F,d_v}$ and they are the query embedding matrix, key embedding matrix, value embedding matrix respectively. $W^O$ is the output matrix which fuse the result from different heads. $d_P$($d_F$) is the dimensionality of $P$($F$), $d_k$ is the embedding dimension of Query/Key, and $d_v$ is the embedding dimension of Value. In this way, model can learn to utilize the position information in aggregating/updating attribute embeddings in a data-driven approach.

Then, after concatenating position embedding and processed attribute embedding, we use a weighted inner production to perform link prediction:
\begin{displaymath}
    \mathcal{A}_{pred} = softmax(\sigma([H_{F} \parallel P]^T \cdot S \cdot [H_{F} \parallel P])).
\end{displaymath}
Here, $S$ is the parameter matrix to be learned. For attribute prediction, we just use a simple two-layer MLP.

%extension: when embedding is at the sub-graph level. Then, each new decoded node need an initial positional embedding[] to get attended context. the afterward process can follow the same steps. the position encoding in the encoder still should be in the input level, correspond to learn a better position info for each sub-graph.

%%when using iterative decoding steps: need both history state and/or initial position embedding to perform context attention

\subsection{Translator Module}
Translator module is a key component in our framework, which is required to build the mapping from the embedding space of source domain to the embedding space of target domain. For paired graphs, this correspondence is easy to be established, by performing a regression task and minimizing the prediction loss. However, for the large amount of unpaired graphs, this kind of training signals can not be obtained. Inspired by ~\cite{belghazi2018mutual,hjelm2018learning}, we propose to use the mutual information score between the source embedding and its translated target embedding as auxiliary supervision to better align these two spaces. As the dimension of embedding space is too high($\mathcal{R}^{N \cdot (d_P+d_F)}$), directly working on it could suffer from curse of dimensionality and result in brittle results. So, we define a $READOUT$ function, which is a global pooling, to fuse the representation of all nodes in a graph. The mutual information score is calculated on top of that, following the same procedures as ~\cite{hjelm2018learning}, which involves a specific estimator. 

For concrete module implementation, we take a simple MLP structure. Here, we perform the translation in a node-wise fashion, and use the global feature along with node-level feature as the input:
\begin{displaymath}
  F_{t} = MLP([F_{s} \parallel P_{s} \parallel READOUT(F_{s},P_{s})]), 
\end{displaymath}
Similar is the case for $P_{t}$. $F_{s}, P_{s}$ is the intermediate node embedding and position embedding in the source domain, and $F_{t}, P_{t}$ are them in the target domain.

\subsection{Adversarial Module}

\subsection{Objective Function of \method}

\subsection{Training Algorithm}
Putting previous parts together, we can get our full model architecture. The optimization goal during training can be written as:
\begin{equation}
\begin{aligned}
  L_{full} = & L_{recon}^{u, p}(G_s,G_s) + L_{recon}^{u, p}(G_t,G_t) \\ & +L_{trans}^{p}([F \parallel P]_{s}, [F \parallel P]_{t}) \\
  & +L_{MI}^{u}(READOUT(F \parallel P)_{s}, READOUT(F \parallel P)_{fake_t}).
\end{aligned}
\end{equation}
$L_{recon}^{u,p}$ is the reconstruction loss for both paired and unpaired graphs, $L_{trans}^{p}$ is the translation loss for paired graphs, and $L_{MI}^{u}$ is the mutual information loss for unpaired graphs. $fake_t$ refers to the generated result in the target domain.

Note that during training, the translation process is supervised only on the intermediate level. During testing, the translation quality is measured at the full graph level, $L_mse(G_t, G_{fake_t})$.

Besides, as our model is composed of multiple different components, we follow a pretrain-finetune pipeline to make the training process more stable. The full training algorithm can be found in Algorithm 1. 

\begin{algorithm}
  \caption{Full Training Algorithm}
  \label{alg:Framwork}
  %\scalebox{0.75}{
  \begin{algorithmic}[1] %???1 ???ÿһ????ʾ??
    \REQUIRE ~~\\ %??????????Input
    $\{\langle G_s, G_t\rangle^p, \langle G_s \rangle^u, \langle G_t\rangle^u \}$.%, and some hyperparameters. 
    \STATE Initialize the encoder, decoder in both source and target domain, by pretraining on loss $L_{recon}^{u, p}$;
    \STATE Fix other parts, only train the translator module, based on loss $L_{trans}^{p}$;
    \STATE Fix the whole model, pretrain the mutual information estimator, following ~\cite{hjelm2018learning};
    \WHILE {Not Converged}
    \STATE Receive a batch of paired graphs $\langle G_s, G_t \rangle^p$; 
    \STATE Update the model using $L_{recon} + L_{trans}$; 
    \STATE Update the multual information estimator;
    \STATE Receive a batch of unpaired graphs $\langle G_s, G_t \rangle^u$;
    \STATE Update the model using $L_{recon} + L_{MI}$; 
    
    \ENDWHILE
  \end{algorithmic}
  %}%% resizebox
\end{algorithm}




==> problem_setting.tex <==
\section{Problem Setting}
We use $G_s = \{\mathcal{V}_{0}, \mathbf{A}_{s}, \mathbf{F}_{s}\}$ to denote an attributed graph from the source domain, where $\mathcal{V}_{0}=\{v_1,\dots,v_N\}$ is a set of $N$ nodes, $\mathbf{A}_{s} \in \mathbb{R}^{N \times N}$ is the adjacency matrix for those nodes. $\mathbf{F}_{s} \in \mathbb{R}^{N \times D}$ denotes the node attribute matrix, where $\mathbf{F}_{s,i} \in \mathbb{R}^{1 \times D}$ is the node attributes of node i and $D$ is the dimension of the node attributes. Similarly, we define the target graph as $G_t = \{\mathcal{V}_{0}, \mathbf{A}_{t}, \mathbf{F}_{t}\}$. In our setting, across different domains, a graph can have different topology and node attributes, but the node set remains the same. On the other hand, different graphs in the same domain are not required to have the same size or the same node sets. For unpaired graph, meaning it is mono-domain and appears only in the source or in the target domain, the dataset can be referred to as $\{G_{s}^{u}, G_{t}^{u}\}$. {$G_{s}^{u}$} refers to the mono-domain graphs in the source side, $G_{t}^{u}$ refers to them in the target side. For paired graph, meaning it is available in both domains, we refer to the dataset as $\{\langle G_s, G_t\rangle\}$. With the above notations, the problem of semi-supervised graph translation is formally defined as
\vskip 0.5em

\noindent{}\textit{Given $\{G_{s}^{u}, G_{t}^{u}, \langle G_s, G_t\rangle \}$, we aim to learn a function $f$ that can transform a source-domain graph to the target domain, i.e.,
%$G(\mathcal{V}_{0}, \mathcal{A}_{s}, \mathcal{F}_{s}) \rightarrow G(\mathcal{V}_{0}, \mathcal{A}_{t}, \mathcal{F}_{t})$,
\begin{equation}
    f(G_s) \rightarrow G_t
\end{equation}
}

